dm_control: Software and Tasks for Continuous Control

The dm_control software package is a collection of Python libraries and task suites for reinforcement learning agents in an articulated-body simulation. A MuJoCo wrapper provides convenient bindings to functions and data structures. The PyMJCF and Composer libraries enable procedural model manipulation and task authoring. The Control Suite is a fixed set of tasks with standardised structure, intended to serve as performance benchmarks. The Locomotion framework provides high-level abstractions and examples of locomotion tasks. A set of configurable manipulation tasks with a robot arm and snap-together bricks is also included. dm_control is publicly available at https://www.github.com/deepmind/dm_control

==> tables/training_steps.tex <==
\begin{tabular}{rrrrrr}
\toprule
        &         &          A3C &          D4PG & D4PG (Pixels) &          DDPG \\
Domain & Task &              &               &                       &               \\
\midrule
acrobot & swingup &   41.9 ± 1.2 &   297.6 ± 8.4 &            81.7 ± 4.4 &    15.4 ± 0.9 \\
        & swingup\_sparse &    0.2 ±  0.1 &   198.7 ± 9.1 &            13.0 ± 1.7 &     1.0 ± 0.1 \\
ball\_in\_cup & catch &  104.7 ± 7.8 &   981.2 ± 0.7 &           980.5 ± 0.5 &   984.5 ± 0.3 \\
cartpole & balance &  951.6 ± 2.4 &   966.9 ± 1.9 &           992.8 ± 0.3 &   917.4 ± 2.2 \\
%        & balance\_sparse &  857.4 ± 7.9 &  1002.0 ± 0.0 &          1002.0 ± 0.0 &   878.5 ± 8.0 \\ ---unmodified---
        & balance\_sparse &  857.4 ± 7.9 &  1000.0 ± 0.0 &          1000.0 ± 0.0 &   878.5 ± 8.0 \\
        & swingup &  558.4 ± 6.8 &   845.5 ± 1.2 &           862.0 ± 1.1 &   521.7 ± 6.1 \\
        & swingup\_sparse &  179.8 ± 5.9 &   808.4 ± 4.4 &          482.0 ± 56.6 &     4.5 ± 1.1 \\
cheetah & walk &  213.9 ± 1.6 &   736.7 ± 4.4 &           523.8 ± 6.8 &   842.5 ± 1.6 \\
finger & spin &  129.4 ± 1.5 &   978.2 ± 1.5 &           985.7 ± 0.6 &   920.3 ± 6.3 \\
        & turn\_easy &  167.3 ± 9.6 &   983.4 ± 0.6 &           971.4 ± 3.5 &   942.9 ± 4.3 \\
        & turn\_hard &   88.7 ± 7.3 &   974.4 ± 2.8 &           966.0 ± 3.4 &   939.4 ± 4.1 \\
fish & swim &   81.3 ± 1.1 &   844.3 ± 3.1 &            72.2 ± 3.0 &   492.7 ± 9.8 \\
        & upright &  474.6 ± 6.6 &   967.4 ± 1.0 &          405.7 ± 19.6 &   854.8 ± 3.3 \\
hopper & hop &    0.5 ± 0.0 &  560.4 ± 18.2 &           242.0 ± 2.1 &   501.4 ± 6.0 \\
        & stand &   27.9 ± 2.3 &   954.4 ± 2.7 &           929.9 ± 3.8 &   857.7 ± 2.2 \\
humanoid & run &    1.0 ± 0.0 &  463.6 ± 13.8 &             1.4 ± 0.0 &   167.9 ± 4.1 \\
        & stand &    6.0 ± 0.1 &   946.5 ± 1.8 &             8.6 ± 0.2 &   642.6 ± 2.1 \\
        & walk &    1.6 ± 0.0 &   931.4 ± 2.3 &             2.6 ± 0.1 &   654.2 ± 3.9 \\
manipulator & bring\_ball &    0.4 ± 0.0 &   895.9 ± 3.7 &             0.5 ± 0.1 &     0.6 ± 0.1 \\
pendulum & swingup &   48.6 ± 5.2 &   836.2 ± 5.0 &          680.9 ± 41.9 &   816.2 ± 4.7 \\
point\_mass & easy &  545.3 ± 9.3 &   977.3 ± 0.6 &           977.8 ± 0.5 &  618.0 ± 11.4 \\
reacher & easy     &   95.6 ± 3.5 &   987.1 ± 0.3 &           967.4 ± 4.1 &   917.9 ± 6.2 \\
        & hard &   39.7 ± 2.9 &   973.0 ± 2.0 &           957.1 ± 5.4 &   904.3 ± 6.8 \\
swimmer & swimmer15 &  164.0 ± 7.3 &  658.4 ± 10.0 &          180.8 ± 11.9 &  421.8 ± 13.5 \\
        & swimmer6 &  177.8 ± 7.8 &  664.7 ± 11.1 &          194.7 ± 15.9 &  394.0 ± 14.1 \\
walker & run &  191.8 ± 1.9 &   839.7 ± 0.7 &          567.2 ± 18.9 &   786.2 ± 0.4 \\
        & stand &  378.4 ± 3.5 &   993.1 ± 0.3 &           985.2 ± 0.4 &   969.8 ± 0.3 \\
        & walk &  311.0 ± 2.3 &   982.7 ± 0.3 &           968.3 ± 1.8 &   976.3 ± 0.3 \\
\bottomrule
\end{tabular}

==> tables/training_time.tex <==
\begin{tabular}{rrrrrr}
\toprule
        &         &           A3C &          D4PG & D4PG (Pixels) &          DDPG \\
Domain & Task &               &               &                       &               \\
\midrule
acrobot & swingup &    64.7 ± 2.0 &   531.1 ± 8.9 &           141.5 ± 6.9 &   149.8 ± 4.2 \\
        & swingup\_sparse &     0.3 ± 0.1 &   415.9 ± 9.5 &            16.3 ± 2.0 &     8.5 ± 0.8 \\
ball\_in\_cup & catch &  643.3 ± 10.9 &   979.8 ± 0.7 &           980.5 ± 0.6 &   984.4 ± 0.3 \\
cartpole & balance &   999.0 ± 0.0 &   982.7 ± 1.4 &           988.3 ± 0.6 &   980.2 ± 0.6 \\
%        & balance\_sparse &  1000.7 ± 0.1 &  1001.7 ± 0.2 &          1002.0 ± 0.0 &   999.4 ± 0.7 \\ ---unmodified---
        & balance\_sparse &  999.7 ± 0.1 &  999.7 ± 0.2 &          1000.0 ± 0.0 &   998.4 ± 0.7 \\
        & swingup &   881.4 ± 0.1 &   836.1 ± 1.6 &           864.0 ± 1.0 &   855.6 ± 0.6 \\
        & swingup\_sparse &   752.5 ± 3.6 &   814.6 ± 0.7 &          649.6 ± 46.9 &   591.1 ± 7.3 \\
cheetah & walk &   519.7 ± 2.2 &   814.6 ± 4.0 &           524.7 ± 6.8 &   849.7 ± 1.7 \\
finger & spin &   446.7 ± 4.2 &   984.7 ± 0.4 &           986.2 ± 0.4 &   916.1 ± 6.3 \\
        & turn\_easy &  291.9 ± 11.3 &   986.1 ± 0.5 &           976.0 ± 1.7 &   927.8 ± 4.9 \\
        & turn\_hard &   200.6 ± 9.6 &   983.2 ± 0.5 &           971.0 ± 2.9 &  618.7 ± 11.8 \\
fish & swim &   395.7 ± 7.3 &   852.5 ± 2.7 &            76.8 ± 4.2 &   666.8 ± 6.8 \\
        & upright &   813.6 ± 4.4 &   971.1 ± 0.9 &          366.8 ± 18.3 &   915.3 ± 2.0 \\
hopper & hop &     0.7 ± 0.1 &  613.2 ± 18.0 &           249.8 ± 2.1 &   435.2 ± 4.9 \\
        & stand &    82.6 ± 5.9 &   956.8 ± 3.9 &           930.0 ± 3.4 &   862.8 ± 2.8 \\
humanoid & run &     1.0 ± 0.0 &   643.1 ± 3.1 &             1.5 ± 0.0 &   137.3 ± 1.3 \\
        & stand &     7.8 ± 0.1 &   959.1 ± 0.8 &             8.7 ± 0.2 &   687.9 ± 2.1 \\
        & walk &     1.7 ± 0.0 &   960.3 ± 0.5 &             2.7 ± 0.1 &   534.4 ± 2.1 \\
manipulator & bring\_ball &     0.6 ± 0.1 &   903.7 ± 3.9 &             0.6 ± 0.1 &     1.2 ± 0.4 \\
pendulum & swingup &    98.8 ± 9.5 &   814.9 ± 5.8 &          705.7 ± 36.7 &   818.6 ± 4.3 \\
point\_mass & easy &   978.5 ± 0.1 &   978.2 ± 0.7 &           979.3 ± 0.3 &   862.3 ± 3.1 \\
reacher & easy     &   285.3 ± 8.9 &   984.9 ± 1.1 &           967.1 ± 4.4 &   969.8 ± 3.0 \\
        & hard &   247.5 ± 9.4 &   982.8 ± 0.4 &           958.0 ± 5.2 &   975.3 ± 0.5 \\
swimmer & swimmer15 &   196.8 ± 8.4 &   681.1 ± 9.3 &          146.0 ± 12.0 &  410.9 ± 10.5 \\
        & swimmer6 &   526.4 ± 9.6 &  651.0 ± 10.0 &          168.9 ± 13.1 &  461.0 ± 10.6 \\
walker & run &   448.4 ± 4.1 &   891.5 ± 5.6 &          566.1 ± 19.1 &   766.5 ± 0.4 \\
        & stand &   707.9 ± 6.5 &   994.0 ± 0.3 &           984.8 ± 0.4 &   973.7 ± 0.3 \\
        & walk &   744.2 ± 2.4 &   983.1 ± 0.4 &           968.1 ± 1.8 &   975.7 ± 0.3 \\
\bottomrule
\end{tabular}

